Harnessing Large Language Models for Seed Generation in Greybox Fuzzing

Greybox fuzzing has emerged as a preferred technique for discovering software bugs, striking a balance between efficiency and depth of exploration. While research has focused on improving fuzzing techniques, the importance of high-quality initial seeds remains critical yet often overlooked. Existing methods for seed generation are limited, especially for programs with non-standard or custom input formats. Large Language Models (LLMs) has revolutionized numerous domains, showcasing unprecedented capabilities in understanding and generating complex patterns across various fields of knowledge. This paper introduces SeedMind, a novel system that leverages LLMs to boost greybox fuzzing through intelligent seed generation. Unlike previous approaches, SeedMind employs LLMs to create test case generators rather than directly producing test cases. Our approach implements an iterative, feedback-driven process that guides the LLM to progressively refine test case generation, aiming for increased code coverage depth and breadth. In developing SeedMind, we addressed key challenges including input format limitations, context window constraints, and ensuring consistent, progress-aware behavior. Intensive evaluations with real-world applications show that SeedMind effectively harnesses LLMs to generate high-quality test cases and facilitate fuzzing in bug finding, presenting utility comparable to human-created seeds and significantly outperforming the existing LLM-based solutions.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

DEV=-dev # To switch dev on
#DEV=

PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf \

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx



samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex${DEV} $(notdir $<); done

samples/sample-sigconf-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex${DEV} $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> tables/magma.tex <==


\begin{table*}[t]
    \vspace{-1.5em}
     \caption{Results of bug-finding evaluation with MAGMA. The numbers stand for the average time-to-trigger of the corresponding bug. Under the same setting, the fuzzing mode producing the shortest time-to-trigger is \colorbox{asparagus}{highlighted} with filled color.}
     \vspace{-1em}
     \label{tab:overall-magma}
     \scriptsize
     \setlength\tabcolsep{5pt}
     \centering
     \begingroup
     \renewcommand{\arraystretch}{1.25}
     % \scalebox{0.9}{
     \begin{tabular}{l|c||c|c|c|c|c|c|c|c|c}
     \hline
     \multirow{2}{*}{\textbf{Project}} & \multirow{2}{*}{\textbf{Bug ID}} & \multicolumn{3}{c||}{{\code{{\sc AFL++}}}} & \multicolumn{3}{c||}{\code{{\sc HONGGFUZZ}}} & \multicolumn{3}{c}{{\code{{\sc AFL}}}}\\ \cline{3-11}
       
       & & \textbf{\tiny Empty} & \textbf{\tiny OSS-FUZZ} & \textbf{\tiny SYS} & \textbf{\tiny Empty} & \textbf{\tiny OSS-FUZZ} & \textbf{\tiny SYS} & \textbf{\tiny Empty} & \textbf{\tiny OSS-FUZZ} & \textbf{\tiny SYS}  \\\hline
    % poppler
       \multirow{2}{*} \sc{POPPLER} & \sc{PDF010} & - & - & \cellcolor{asparagus}{\code{21m}} & -  &  - & -   & -  & - & \code{7h}    \\

       & \sc{PDF016}  & \code{24m} & - & \cellcolor{asparagus}{\code{28s}}  & -  &  \code{6m} & \code{40s}   & \code{14m}  & \code{1m} & \code{13m}  \\\cline{1-11}
       
       % libxml
       \multirow{2}{*}\sc{LIBXML2} & \sc{XML009} & \code{4d} & \code{1h} & \cellcolor{asparagus}{\code{10s}} & \code{4d}  &  \code{2m} & \code{28s}   & \code{1w}  & \code{2h} & \code{11m}    \\
       
       & \sc{XML017}  & \code{4d} & \code{4d} & \code{2d}  & \code{5h}  &  \code{9h} & \code{2d}   & \code{4d}  & \code{4d} & \code{1w}  \\\cline{1-11}
      
     \bottomrule
     \end{tabular}
     \endgroup
     \label{-3.75em}
   \end{table*}
   

==> tables/projects.tex <==
\begin{table}[]
\setlength\tabcolsep{4pt}
\centering
\begin{tabular}{l|l}
\hline
\textbf{Project Name} & \textbf{\# of Harness Binaries} \\ \hline
{\sc arduinojson } & 2 \\
\hline
{\sc arrow } & 4 \\
\hline
{\sc avahi } & 6 \\
\hline
{\sc bignum-fuzzer } & 4 \\
\hline
{\sc bind9 } & 11 \\
\hline
{\sc binutils } & 25 \\
\hline
{\sc bloaty } & 1 \\
\hline
{\sc boringssl } & 2 \\
\hline
{\sc brpc } & 10 \\
\hline
{\sc cairo } & 5 \\
\hline
{\sc c-ares } & 2 \\
\hline
{\sc c-blosc } & 2 \\
\hline
{\sc c-blosc2 } & 1 \\
\hline
{\sc cgif } & 1 \\
\hline
{\sc circl } & 1 \\
\hline
{\sc cjson } & 1 \\
\hline
{\sc cpp-httplib } & 1 \\
\hline
{\sc croaring } & 1 \\
\hline
{\sc crow } & 2 \\
\hline
{\sc curl } & 4 \\
\hline
{\sc cyclonedds } & 4 \\
\hline
{\sc dng\_sdk } & 5 \\
\hline
{\sc dropbear } & 6 \\
\hline
{\sc exiv2 } & 1 \\
\hline
{\sc ffmpeg } & 4 \\
\hline
{\sc file } & 2 \\
\hline
{\sc fio } & 1 \\
\hline
{\sc flac } & 9 \\
\hline
{\sc gdbm } & 1 \\
\hline
{\sc gfwx } & 2 \\
\hline
{\sc giflib } & 2 \\
\hline
{\sc gnutls } & 4 \\
\hline
{\sc grok } & 1 \\
\hline
{\sc guetzli } & 1 \\
\hline
{\sc h2o } & 4 \\
\hline
{\sc hoextdown } & 1 \\
\hline
{\sc hpn-ssh } & 7 \\
\hline
{\sc igraph } & 4 \\
\hline
{\sc imagemagick } & 4 \\
\hline
{\sc inih } & 1 \\
\hline
{\sc jansson } & 1 \\
\hline
{\sc jbig2dec } & 1 \\
\hline
{\sc jq } & 6 \\
\hline
{\sc kcodecs } & 1 \\
\hline
{\sc knot-dns } & 4 \\
\hline
{\sc krb5 } & 11 \\
\hline
{\sc lame } & 1 \\
\hline
{\sc lcms } & 12 \\
\hline
{\sc leptonica } & 7 \\
\hline
{\sc libarchive } & 1 \\
\hline
{\sc libbpf } & 1 \\
\hline
{\sc libdwarf } & 5 \\
\hline
{\sc libexif } & 2 \\
\hline
{\sc libfido2 } & 5 \\
\hline
{\sc libgd } & 8 \\
\hline
{\sc libheif } & 4 \\
\hline
{\sc libical } & 2 \\
\hline
{\sc libidn } & 3 \\
\hline
{\sc libidn2 } & 3 \\
\hline
{\sc libjpeg-turbo } & 4 \\
\hline
{\sc liblouis } & 3 \\
\hline
{\sc libmodbus } & 2 \\
\hline
{\sc libplist } & 4 \\
\hline
{\sc libpsl } & 6 \\
\hline
{\sc libraw } & 4 \\
\hline
{\sc libreoffice } & 3 \\
\hline
{\sc libspng } & 3 \\
\hline
{\sc libsrtp } & 1 \\
\hline
{\sc libssh } & 5 \\
\hline
{\sc libtasn1 } & 5 \\
\hline
{\sc libtiff } & 1 \\
\hline
{\sc libtorrent } & 3 \\
\hline
{\sc libtpms } & 1 \\
\hline
{\sc libxls } & 1 \\
\hline
{\sc libxlsxwriter } & 1 \\
\hline
{\sc libxml2 } & 8 \\
\hline
{\sc libxslt } & 2 \\
\hline
{\sc libyal } & 20 \\
\hline
{\sc libyaml } & 8 \\
\hline
{\sc libzip } & 4 \\
\hline
{\sc libzmq } & 1 \\
\hline
{\sc llamacpp } & 2 \\
\hline
{\sc lldpd } & 4 \\
\hline
{\sc lua } & 3 \\
\hline
{\sc lwan } & 5 \\
\hline
{\sc lzma } & 8 \\
\hline
{\sc lzo } & 3 \\
\hline
{\sc matio } & 1 \\
\hline
{\sc mbedtls } & 12 \\
\hline
{\sc mdbtools } & 1 \\
\hline
{\sc mercurial } & 4 \\
\hline
{\sc miniz } & 8 \\
\hline
{\sc minizip } & 1 \\
\hline
{\sc monero } & 1 \\
\hline
{\sc mosh } & 2 \\
\hline
{\sc ms-tpm-20-ref } & 1 \\
\hline
{\sc mupdf } & 1 \\
\hline
{\sc ndpi } & 16 \\
\hline
{\sc neomutt } & 1 \\
\hline
{\sc nestegg } & 1 \\
\hline
{\sc net-snmp } & 1 \\
\hline
{\sc ninja } & 1 \\
\hline
{\sc nokogiri } & 1 \\
\hline
{\sc ntopng } & 1 \\
\hline
{\sc ntpsec } & 3 \\
\hline
{\sc open62541 } & 5 \\
\hline
{\sc opendnp3 } & 2 \\
\hline
{\sc openjpeg } & 1 \\
\hline
{\sc opennavsurf-bag } & 2 \\
\hline
{\sc opensc } & 12 \\
\hline
{\sc openssh } & 5 \\
\hline
{\sc openvswitch } & 6 \\
\hline
{\sc openweave } & 6 \\
\hline
{\sc opus } & 2 \\
\hline
{\sc p11-kit } & 1 \\
\hline
{\sc pcapplusplus } & 5 \\
\hline
{\sc pffft } & 2 \\
\hline
{\sc picotls } & 2 \\
\hline
{\sc pjsip } & 12 \\
\hline
{\sc powerdns } & 7 \\
\hline
{\sc pugixml } & 2 \\
\hline
{\sc pupnp } & 1 \\
\hline
{\sc qpdf } & 6 \\
\hline
{\sc qpid-proton } & 2 \\
\hline
{\sc qt } & 2 \\
\hline
{\sc qubes-os } & 5 \\
\hline
{\sc rabbitmq-c } & 3 \\
\hline
{\sc rapidjson } & 1 \\
\hline
{\sc readstat } & 11 \\
\hline
{\sc rnp } & 8 \\
\hline
{\sc s2opc } & 4 \\
\hline
{\sc selinux } & 3 \\
\hline
{\sc simdjson } & 6 \\
\hline
{\sc skcms } & 3 \\
\hline
{\sc sleuthkit } & 10 \\
\hline
{\sc spdlog } & 5 \\
\hline
{\sc spirv-tools } & 6 \\
\hline
{\sc stb } & 2 \\
\hline
{\sc strongswan } & 7 \\
\hline
{\sc sudoers } & 8 \\
\hline
{\sc tarantool } & 5 \\
\hline
{\sc tinyusb } & 3 \\
\hline
{\sc tmux } & 1 \\
\hline
{\sc tomlplusplus } & 1 \\
\hline
{\sc tor } & 16 \\
\hline
{\sc unbound } & 4 \\
\hline
{\sc unit } & 5 \\
\hline
{\sc usbguard } & 3 \\
\hline
{\sc utf8proc } & 1 \\
\hline
{\sc util-linux } & 4 \\
\hline
{\sc valijson } & 1 \\
\hline
{\sc wasmedge } & 2 \\
\hline
{\sc wavpack } & 1 \\
\hline
{\sc wget } & 10 \\
\hline
{\sc wireshark } & 4 \\
\hline
{\sc woff2 } & 2 \\
\hline
{\sc wolfssl } & 3 \\
\hline
{\sc wt } & 4 \\
\hline
{\sc wuffs } & 10 \\
\hline
{\sc wxwidgets } & 1 \\
\hline
{\sc xz } & 3 \\
\hline
{\sc yajl-ruby } & 1 \\
\hline
{\sc yara } & 6 \\
\hline
{\sc zlib } & 9 \\
\hline
{\sc zlib-ng } & 7 \\
\hline
{\sc zstd } & 2 \\
\hline

\end{tabular}
\caption{Harness Binaries Grouped by Project}
\end{table}

